Programming and Deployment of Autonomous Swarms using Multi-Agent Reinforcement Learning

Autonomous systems (AS) carry out complex missions by continuously observing the state of their surroundings and taking actions toward a goal. Swarms of AS working together can complete missions faster and more effectively than single AS alone. To build swarms today, developers handcraft their own software for storing, aggregating, and learning from observations. We present the Fleet Computer, a platform for developing and managing swarms. The Fleet Computer provides a programming paradigm that simplifies multi-agent reinforcement learning (MARL) -- an emerging class of algorithms that coordinate swarms of agents. Using just two programmer-provided functions Map() and Eval(), the Fleet Computer compiles and deploys swarms and continuously updates the reinforcement learning models that govern actions. To conserve compute resources, the Fleet Computer gives priority scheduling to models that contribute to effective actions, drawing a novel link between online learning and resource management. We developed swarms for unmanned aerial vehicles (UAV) in agriculture and for video analytics on urban traffic. Compared to individual AS, our swarms achieved speedup of 4.4X using 4 UAV and 62X using 130 video cameras. Compared to a competing approach for building swarms that is widely used in practice, our swarms were 3X more effective, using 3.9X less energy.

==> Background.tex <==
\section{Background}
\label{sect:background}



\begin{comment}
\begin{figure*}[t]
 \centering
  \includegraphics[scale=0.9]{figures/TypesofAutonomy.pdf}
 \caption{Automated and Autonomous robots differ in their capabilities, with autonomous robots capable of making complex decisions. Autonomated and autonomous robots can swarm, augmenting their ability to accomplish tasks and navigate complex environments.}
  \label{fig:autonomy-types}
\end{figure*}
\end{comment}
Autonomous systems operate above and beyond the capabilities of conventional robots. They sense and respond to their environment, solve well or poorly defined problems, and are often capable of complex decision-making~\cite{fahimi2009autonomous}. Considerable work has been done in the past decade to advance autonomous robots. Self-driving cars~\cite{lin2018architectural, urmson2008autonomous}, autonomous aerial vehicles~\cite{boubin2019managing,sanchez2016aerostack,zhang2012application}, and smaller autonomous terrestrial robots~\cite{siegwart2011introduction,pfeiffer2017perception,bouman2020autonomous} have a number of uses in industry and research. Self driving vehicles have received considerable attention over the past decade, resulting in a \$56 billion dollar ~\cite{uavmarket2020} industry and an active research community. Autonomous UAV, to a lesser extent, have received industry and military attention for package and food delivery, aerial photography, infrastructure inspection, and surveillance~\cite{primeair,boubin2019managing,al2017vbii,semsch2009autonomous}. Smaller terrestrial robots are also of interest for short distance deliveries, customer service, data collection, and more~\cite{arbanas2016aerial,amazonscout,mueller2017robotanist,niemela2017social}. 

Due to power, compute, and range limitations, it is often advantageous for autonomous robots to work together to accomplish tasks. Groups of cooperative robots are referred to as swarms~\cite{nouyan2008path}. Robot swarms, particularly swarms of autonomous robots, have the potential to revolutionize a number of industries and applications. Interconnected autonomous vehicles have the potential to eliminate accidents and traffic slowdowns~\cite{gora2016traffic}. 
UAV swarms have also attracted mainstream attention through the impressive 3D swarm-based light shows~\cite{kshetri20182018}. Swarms are, in fact, a mature idea~\cite{campion2018review} with a number of research implementations and industry developments. Swarms of automated and autonomous UAV for military applications~\cite{sanders2017drone}, agriculture~\cite{ju2018multiple,albani2017monitoring}, search and rescue~\cite{arnold2020heterogeneous}, infrastructure inspection~\cite{shakhatreh2019unmanned}, and delivery~\cite{primeair} among other domains are in various stages of development. 

Development of application specific autonomous robots and swarms, particularly when using UAV, is challenging. UAV require the capability to sense and perceive their surroundings and plan routes and actions to accomplish goals on a tight power and compute budget~\cite{campion2018review}. Due to recent advancements in artificial intelligence, robotic perception and image processing have improved considerably in the past decade. Object detectors and image segmentation techniques have become easier to develop, train, and tune with modern software toolkits~\cite{abadi2016tensorflow}, and off-the-shelf solutions often exist for common problems like facial recognition~\cite{boyko2018performance}. Despite the increased availability of accurate object detectors, many problems applicable to autonomous UAV, like agricultural scouting, often require bespoke models where data availability is poor. Swarms introduce further complications. Object detection is a complex workload and can consume considerable power and compute resources, which are scarce onboard UAV. If compute must be offloaded to the edge or cloud, compute resources and power budgets will increase with the size of the swarm. Provisioning edge resources, networks, sensors, and power in areas where swarms and autonomous systems operate can prove challenging~\cite{vasisht2017farmbeats}. 

Pathfinding for autonomous UAV swarms is also incredibly important. The goal of robotic pathfinding is to determine which data to next sense in order to most quickly and effectively accomplish the systems autonomy goals. Robots usually maintain a map of all possible waypoints within a region, which the path finding system must select from. Path finding methods use a number of techniques like mutual information~\cite{julian2014mutual} and rapid exploration~\cite{cui2015mutual} in an attempt to make the best possible decision using limited information, but these mechanisms, while often returning an optimal result, can be slow. Autonomous UAV, are highly resource constrained. Battery lives are often less than 25 minutes, with most of the battery capacity going to motor thrust. Algorithms that require considerable exploration will burn UAV battery quickly. Fast path finding with some inaccuracy is preferred to highly accurate but slow pathfinding. For these reasons, reinforcement learning has been adopted, replacing live sensing with the use of profile data from prior executions.

Reinforcement learning pathfinding for autonomous UAV relies on a two key factors: feature extraction and feature matching~\cite{boubin2019autonomic,zhang2020}. Autonomous UAV extract features from sensed data that are relevant to current autonomy goals. These may be as complex as locations or numbers of objects in images, or as simple as pixel-based insights like vegetation index. Once features are extracted on-board or at the edge, reinforcement learning compares data from a large number of prior examples to determine best actions. Past samples with similar features are examined to determine their highest utility actions. A consensus of these images determines the next action of the FAAS. The utility of a FAAS action is based on its progression towards a goal, with positive values indicating forward progress. Utility is calculated based on actions with a local map, which means the global utility (affect on the entire swarm) of an action and local utility (affect on the local swarm) may not align. 

Reinforcement learning methods for autonomous UAV are young, and could benefit from improvement. For instance reinforcement learning could benefit from prior work in online learning~\cite{hasler2018interactive} and federated learning for autonomous systems~\cite{yang2019federated}. Online learning describes the process of continually retraining models in execution. Instead of relying only on prior datasets, autonomous UAV may gain key insights from very recent execution data. In a large swarm, online learning may prove difficult. Online model retraining may be compute and network intensive, requiring data movement and compute resources above and beyond normal inference. Federated learning, the process of combining locally trained models into a globally accurate model across a distributed system, could greatly benefit swarm pathfinding. Swarm members working on the same task may benefit from the data each senses. Members may also be geographically distributed, with highly constrained networks, complicating data and model movement. Early work has been done on adding federated learning to UAV swarms and autonomous robots~\cite{zeng2020federated,shiri2020communication,li2020review, hasler2018interactive}, but not yet as part of an end to end solution.

Given the power, networking, model creation, and pathfinding problems autonomous aerial swarms face, we believe an end to end solution to swarm building is the next logical step in adoption. The Fleet Computer is this solution. The fleet computer provides a programming model for developing and debugging object detection models and autonomy goals for swarms of autonomous robots. It uses online federated learning to improve pathfinding across the swarm with minimal data movement. The fleet computer can be easily expanded and contracted, allowing addition, removal, and duty cycling of compute resources as demand changes to efficiently use available power. The fleet computer introduces the first end to end software architecture for UAV swarm development and deployment. In this paper, we describe the fleet computer, its implementation, and its performance.

In section 3 of this paper, we describe the fleet computer's architecture. Section 4 covers the fleet computers programming model. Section 5 outlines online learning within the fleet computer programming model. Section 6 discusses the fleet computer's implementation, Sections 7 and 8 cover the fleet computer's performance results and discussion. 

\begin{figure}[t]
 \centering
  \includegraphics[scale=0.23]{figures/ComparisonTable.png}
 \caption{Automated and Autonomous robots differ in their capabilities, with autonomous robots capable of making complex decisions. Autonomated and autonomous robots can swarm, augmenting their ability to accomplish tasks and navigate complex environments.}
  \label{fig:autonomy-types}
\end{figure}

\begin{comment}

This method poses a series of problems for large scale systems. First, the amount of profile data available to these systems can be enormous (on the order of Terabytes or larger of images and extracted features). Full datasets are often too large for edge systems to search through in real-time, so datasets must be broken down, leaving potentially relevant data on the table. Second, reinforcement learning path finding relies on data sensed at runtime to inform future decisions. Adding data from the current execution into the reinforcement learning data set at runtime can provide meaningful insights. UAV from different edge systems (and thus different data sets) may be operating in similar geographic areas, meaning information shared on one edge system may positively inform operations on another.

Swarms and their compute resources may be geographically distributed

To solve these problems, data must be shareable between edge nodes in distributed swarms for federated learning~\cite{yang2019federated}. FAAS designs often maintain access to the cloud for offloading machine learning tasks. We propose that the cloud component of FAAS be used for path finding as well. In this new distributed system, edge and cloud will combine to, dynamically allocate resources for retraining pathfinding models based on data shared between edge systems.

Prior FAAS Pathfinding methods use A* search or K-Nearest-Neighbors (KNN) to approximate the utility of future FAAS motions given the similarity of prior data samples~\cite{boubin2019managing}. This approach relies heavily on data either provided to the local system, or that the local system has collected in execution. For an FAAS swarm, two naive approaches emerge. First, implementers could periodically combine all data and retrain the model as a batch, distributing the new model to swarm-members upon completion. Second, local models could be retrained using only data they collected. The first naive approach assumes that either all data captured by all swarm members is useful to all other swarm members, or that data that is not useful to some or all swarm members will be disregarded, neither of which can be easily guaranteed. It also does not account for data-movement costs. FAAS may have high data-movement costs to the cloud or between base-stations, so requiring total data centralization for any update could slow or totally preclude updates. The second naive approach does not require data-movement, but leaves data on the table. Swarm members may be sensing data that can inform other members pathfinding approaches; however, this is not guaranteed. A balanced approach must be found.

To balance these competing requirements, we propose training group of models using a network and model-quality aware approach to federated learning. This method involved 3 facets: 1) a set of models to be trained, each on a different combination of data sensed from edge systems, 2) an online hyperparameter optimization mechanism for determining the usefulness of a model to pathfinding, and 3) a network and model-utility aware scheduling algorithm for model training across edge and cloud. 

Because we can not be sure which sensed data will be useful, neutral, or detrimental to reinforcement learning before training, multiple models should be trained concurrently with a combination of data from different edge systems. Each model should then be checked for pathfinding decisions, and their results combined and weighted based on the predetermined value of prior predictions from that model. We propose that the number of models be equal to the powerset of all edge systems sensing data, with the null-set model consisting of the initial input model. This will provide each edge system with models trained on every combination of edge system data, allowing it to determine online how useful those models are to its pathfinding. 

Usefulness in the context of a set of RL pathfinding models can be viewed as its own meta-model, consisting of one hyper-parameter per model used to weight the prediction of said input model. The output of this meta-model should be a pathfinding decision. The goal of our approach is to find the set of usefulness weights that returns the best pathfinding result. This constitutes an online hyperparameter tuning problem~\cite{tang2020online,zhan2018efficient}, a relatively new area. We propose using Bayesian optimization~\cite{bergstra2013hyperopt}, a tried and tested hyperparameter optimization approach, to optimize our usefulness function.

By determining the usefulness of a model, we can infer that updates to models with high usefulness values will have a larger impact on FAAS pathfinding, and should receive priority access to resources. Model updates should therefore be scheduled at least in part based on their usefulness. Model retraining must also be managed across the edge and cloud, balancing usefulness and network latency with overall update speed. Using Kubernetes~\cite{burns2016borg}, a distributed container orchestration system, we can schedule containers based on usefulness, while also accounting for data-movement.

Figure ~\ref{fig:design-draw} shows this paradigm. A series of models are assigned to different edge and cloud systems for training, updating models at the edge periodically. Over a mission, the edge system controlling a UAV determines the usefulness ($U_i$) of that model through Bayesian optimization, and returns the usefulness value to Kubernetes. Kubernetes, in turn, reschedules that model (potentially on another edge system) and provides the scheduling priority ($P_i$) of that model to the node on which it trains, allowing that node to allocate resources to that model accordingly.


Through the rest of this paper, we describe how we leverage Kubernetes' robust scheduler, along with our own priority scheme and reinforcement learning algorithms to create an FAAS swarm with online learning capabilities. Section 3 of this paper describes the design of this system, Section 4 presents implementation details, and Section 5 shows results gathered from real FAAS missions capturing crop yield in corn fields and surveying crumbling infrastructure for faults. 


\iffalse
checking the performance of edge systems and periodically updating their local data sets to maximize global utility. This involved several systemic changes to prior FAAS: 1) maintaining the entire reinforcement learning data set in the cloud, 2) updating the full data set throughout FAAS execution, 3) comparing utility differences between local pathfinding (at the edge) to global pathfinding (in the cloud using the entire data set), and 4) dispatching updates to local data sets to improve utility. 

To implement this system, the governor must have access to the entire reinforcement learning data set, which may Terabytes in size or larger. This master data set must be accessible to FAAS edge system, who will commit updates after each path finding decision. The governor will maintain a global map, containing all FAAS positions and movements, which will be updated with each commit. The global utility of each committed flight action will also be calculated, requiring the governor to perform a second, after the fact, path finding analysis. 

Local FAAS actions may (due to lack of data) produce results that reduce or do not optimally increase global utility. If the governor determines that an edge system has made a significant number of under-performing flight actions, the local data set of this system should be updated. The governor should transfer data to the local system, replacing its least effective data entries with the entries that informed the maximum-utility decisions of the governor. This architecture assures that edge systems inevitably work toward global utility without the need for expensive and high power storage and processing units to maintain global maps and data sets. 
This does, however, put pressure on networks. NormKubernetes  [22],  a  distributed  container  orchestrational FAAS require only WiFi connection between UAV and the edge, and potentially a cellular or TVWS connection between the edge and cloud. 

For FAAS to quickly upload and download large amounts of data to and from the cloud, modern networking advancements will be needed. 5G technologies like virtual radio access networks must be leveraged to assure that large (on the order of Gigabytes) updates can be quickly transferred to edge systems to influence path finding decisions. This solution requires the deployment of one or more 5G small cells to cover the FAAS edge system controlling the swarm. 

To best utilize 5G networks, a SDN should facilitate communication between edge and cloud. Uploads from FAAS to the cloud are quite small, but downloads of information from cloud to edge could be as large as the replacement of an entire local dataset. Moreover, FAAS must continue making decisions while reinforcement learning datasets are updating, and may therefore make decisions based on only partially updated datasets. When relying on cellular networks, FAAS must also consider variabilities in network traffic which may periodically slow upload or download speed. To mitigate the negative consequences of these factors, A SDN between cloud and edge will determine when cloud and edge updates should occur based on network throughput and which data points are replaced in local datasets throughout the update process. Our SDN design focuses on the governor as a centralized control point. 

Future work on this project requires the implementation of this system. FAAS have been conclusively implemented with the open source software SoftwarePilot~\cite{SoftwarePilot}. We plan to modify this system by implementing the cloud governor described along with software defined networking capabilities to take full advantage of 5G networks.
\fi

\end{comment}
